Where to Encode: A Performance Analysis of x86 and Arm-based Amazon EC2 Instances

Video streaming became an undivided part of the Internet. To efficiently utilize the limited network bandwidth it is essential to encode the video content. However, encoding is a computationally intensive task, involving high-performance resources provided by private infrastructures or public clouds. Public clouds, such as Amazon EC2, provide a large portfolio of services and instances optimized for specific purposes and budgets. The majority of Amazon instances use x86 processors, such as Intel Xeon or AMD EPYC. However, following the recent trends in computer architecture, Amazon introduced Arm-based instances that promise up to 40% better cost-performance ratio than comparable x86 instances for specific workloads. We evaluate in this paper the video encoding performance of x86 and Arm instances of four instance families using the latest FFmpeg version and two video codecs. We examine the impact of the encoding parameters, such as different presets and bitrates, on the time and cost for encoding. Our experiments reveal that Arm instances show high time and cost-saving potential of up to 33.63% for specific bitrates and presets, especially for the x264 codec. However, the x86 instances are more general and achieve low encoding times, regardless of the codec.

==> sections/deleted.tex <==
%Therefore, the cloud providers offer instances, which have been optimised for video transcoding~\cite{Li:2019}. %For example, Amazon EC2 provides instance families, based on different processor architecture with a main goal to improve the execution time for video transcoding.
%each optimized for specific purposes~\cite{Li:2019} (i. e. the balanced general purpose \texttt{m} instances, the compute-optimized \texttt{c} instances, the memory-optimized \texttt{r} instances, and the burstable \texttt{t} instances). Currently, some of the leading video transcoding companies also use different types of EC2 Spot Instances for video transcoding~\cite{Amazon:2017}.

%To support efficient video transcoding, Amazon recently released their second generation Graviton \texttt{\acrshort{arm}}-based processors. Graviton2 is a 64-core monolithic server chip design and uses \acrshort{arm}’s new Neoverse N1 cores, which is a derivation of the mobile Cortex-A76 cores. With the second generation of Graviton, Amazon EC2 promises higher performance at lower cost, compared to traditional Intel Xeon instances with \texttt{x86} architecture. %For example, Graviton2 instances, such as \texttt{m6g}, \texttt{c6g}, and \texttt{r6g} provide up to $40\%$ better price performance over comparable instance types with Intel Xeon processor for a broad spectrum of workloads~\cite{AmazonGraviton2}. 
%First, we draw several insights from the comparison of instances of the same family with different processor architecture. Second, we present the fastest instance type per processor architecture for each encoding experiment. Third, we analyse how the encoding performance changes with increasing number of threads.

\paragraph{Encoding data generation}
\begin{itemize}
\item \emph{Video sequence selection} encompasses the selection of a raw video segment for encoding;
\item \emph{Codec selection} involves the identification of representative codecs, widelly used in industry and research;
\item \emph{Encoding parameters selection} includes the identification the stream bitrate, the video resolution and the quality to speed ratio.   
\end{itemize}

\paragraph{Performance evaluation}
\begin{itemize}
\item \emph{Instance type} identification includes the selection of appropriate VM instances most commonly used for video encoding;
\item \emph{Computer architecture} encloses the identification of microprocessor architecture for the selected instance types;  
\item \emph{Evaluation metrics} includes identification of performance metrics in terms of encoding time, scalability and induced financial costs. 
\end{itemize}

%methods to predict the transcoding performance of different cloud computing units for the optimal scheduling of video transcoding tasks with multiple codecs and transcoding parameters in a heterogeneous cloud infrastructure.



%Thereafter, from the speedup $S$ we derive the efficiency $E$ as: 
%\begin{equation}
%E = \frac{S}{N_{vCPU}},
%\end{equation}
%where $N_{vCPU}$ is the number of vCPUs provided by the instance.
%s\roland{The efficiency is not yet in the results}

% I replace this for now, but maybe we need it later
%\subsubsection{Cost-performance ratio}
%We define the \textit{Cost-performance ratio} $C_r$ as:
%\begin{equation}
%C_r = \frac{t_{Arm}(V_{b,p})*c_{Arm}}{t_{x86}(V_{b,p})*c_{x86}}.
%\end{equation}
%where $c_{Arm}$ is the cost of the \texttt{\acrshort{arm}} instance, $c_{x86}$ is the cost of the \texttt{x86} instance. 

%   a value $\geq 1$ indicates that the \texttt{\acrshort{arm}} instance has better cost-performance ration than the reference \texttt{x86} instance.

==> sections/old_texts.tex <==
%This means that on the \texttt{\acrshort{arm}} instances, one vCPU is assigned to a single physical core, while on the  \texttt{x86} instances two vCPUs are served by a single physical core with a thread level parallelism.
%\paragraph{Speedup} of \texttt{\acrshort{arm}} and \texttt{x86} instances with respect to the number of execution threads. We use the speedup as a metric to identify how the \texttt{\acrshort{arm}} instances compare to the \texttt{x86}, which are based on processors that utilize thread level parallelism (hyper-threading technology) to increase the overall execution efficiency. More concretely, for all \texttt{x86} instances except the \texttt{t2}, each vCPU is by default a hyper-thread of an Intel Xeon core, i.e., one vCPU corresponds to one hyper-threaded logical core~\cite{opt-cpu-options}. In contrast, \texttt{\acrshort{arm}} instances assign one vCPU to a one physical core. This means that on the \texttt{\acrshort{arm}} instances, one vCPU is assigned to a single physical core, while on the  \texttt{x86} instances two vCPUs are served by a single physical core with a thread level parallelism. Therefore, to identify how the utilization of thread level parallelism influences the encoding execution, we explore the scalability potential of the \texttt{\acrshort{arm}} and \texttt{x86} instances for increased number of execution threads with a fixed number of vCPUs. 

%We quantify the variation of the encoding time per instance type with the increasing the number of execution threads over fixed number of available vCPUs using the speedup metric: 
%\begin{equation}
%S = \frac{t_{r
%}(V_{b,p})}{t_{e}(V_{b,p})},
%\end{equation}
%where $t_{r}$ is the reference encoding time with a reference number of threads and $t_{e}$ is the scaled encoding time with a scaled number of threads. The reference number of threads $r$ is equal to the available vCPUs. The scaled number of threads $e = r \cdot 2 $ corresponds to the number of hyper-threads supported per physical core by the Intel Xeon processor.   



%For the scalability evaluation, we identify the $t_{r}=8$ in relation to the available vCPUs of the selected instances~\cite{Lee:2020}. Furthermore, we select $t_{e}=t_{r}\cdot2$ to evaluate the performance of the instances in cases where the number of execution threads is higher than the number of available vCPUs. We select the specific value for $t_{e}$ as the \texttt{x86} instances for our evaluation assign by default two threads per physical core.     

%The TI metric shows the amount of motion between frames in a video sequence and SI metric reflects the spatial complexity of a video content, as
